Encoding Optimization for Low-Complexity Spiking Neural Network Equalizers in IM/DD Systems

Neural encoding parameters for spiking neural networks (SNNs) are typically set heuristically. We propose a reinforcement learning-based algorithm to optimize them. Applied to an SNN-based equalizer and demapper in an IM/DD system, the method improves performance while reducing computational load and network size.

==> figures/ber_arnold.tex <==
\begin{tikzpicture}[thick,>=latex]


    \begin{axis}[
        width=.45\textwidth,
        height=.2\textwidth,
        ymode = log,
        xscale=1,
        ylabel={$\mathrm{BER}$},
        xtick = {2,4,6,8,10},
        grid=major,
        legend cell align={left},
        legend style={
            at={(0.98,0.98)},
            anchor=north east,
            fill opacity = 0.8,
            draw opacity = 1, 
            text opacity = 1,
        },
        xmin=4,xmax=10,
        ymin=3e-4,ymax=2e-3,
        axis line style=thick,
        tick label style={/pgf/number format/fixed},
        xticklabels = {},
        ytick = {3e-4,4e-4,5e-4,6e-4,7e-4,8e-4,9e-4,1e-3,2e-3},
        yticklabels = {$\num{0,0003}$,,,,,,,$\num{0,001}$,$\num{0,002}$},
        ]   

    \addplot[color=KITcyanblue, line width=\lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax4_ber] {figures/txt/arnold.txt};
    \addplot[color=KITorange, line width=\lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax6_ber] {figures/txt/arnold.txt};
    \addplot[color=KITpalegreen, line width=\lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax8_ber] {figures/txt/arnold.txt};
    \addplot[color=KITpurple, line width=\lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax10_ber] {figures/txt/arnold.txt};
    \addplot[color=black, dashed, line width = \lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax60_noopt_ber] {figures/txt/arnold.txt};
    
    


    \addplot[color=gray, dashed, line width = \lwidth,mark=*,mark size=\marksz,mark options={solid}] coordinates {(1, 8e-4) (10, 8e-4)};

    \end{axis}
\end{tikzpicture}


==> figures/mac.tex <==
\begin{tikzpicture}[thick,>=latex]
    \def\lwidth{1.0}
    \def\opac{100}
    \def\opaci{100}
    \def\marksz{1.5pt}

    \begin{axis}[
        axis x line = bottom,
        axis line style={-},         %
        thick,   
        ymode = log,                    
        width=.45\textwidth,
        height=.25\textwidth,
        xscale=1,
        xlabel=$J$,
        ylabel={\#MAC},
        xtick = {2,4,6,8,10},
        grid=major,
        legend cell align={left},
        legend style={
            at={(0.5,1.1)},
            anchor=south,
            fill opacity = 0.8,
            draw opacity = 1, 
            text opacity = 1,
            legend columns=3,
            /tikz/every even column/.append style={column sep=.1cm},
            scale=.8
        },
        legend image post style={xscale=0.5, yscale=0.5},
        xmin=4,xmax=10,
        ymin=1e3,ymax=1e6,
        axis line style=thick,
        tick label style={/pgf/number format/fixed},
        after end axis/.code={
        \draw[line width=1pt] (rel axis cs:-0.003,1) -- (rel axis cs:1.003,1); %
        \draw[line width=1pt] (rel axis cs:-0.003,0) -- (rel axis cs:1.003,0); %
    }
        ]
    
    \addlegendimage{solid,color=KITcyanblue,line width=\lwidth}\addlegendentry{$K=4$}
    \addlegendimage{solid,color=KITorange,line width=\lwidth}\addlegendentry{$K=6$}
    \addlegendimage{solid,color=KITpalegreen,line width=\lwidth}\addlegendentry{$K=8$}
    \addlegendimage{solid,color=KITpurple,line width=\lwidth}\addlegendentry{$K=10$}
    \addlegendimage{dashed, color=gray, line width=\lwidth} \addlegendentry{$\mathrm{ref}$}
    \addlegendimage{dashed,color=black,line width=\lwidth}\addlegendentry{$K=60,\, \mathrm{NoOpt}$}
    

    \addplot[color=KITcyanblue, line width=\lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax4_mac] {figures/txt/arnold.txt};
    \addplot[color=KITorange, line width=\lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax6_mac] {figures/txt/arnold.txt};
    \addplot[color=KITpalegreen, line width=\lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax8_mac] {figures/txt/arnold.txt};
    \addplot[color=KITpurple, line width=\lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax10_mac] {figures/txt/arnold.txt};
    \addplot[color=black, dashed, line width = \lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax60_noopt_mac] {figures/txt/arnold.txt};
    
    \addplot[color=gray, dashed, line width = \lwidth,mark=*,mark size=\marksz,mark options ={solid}] coordinates {(1, 177600) (10, 177600)};
    

    \end{axis}


\end{tikzpicture}


==> figures/spike_rate.tex <==
\begin{tikzpicture}[thick,>=latex]
    \def\lwidth{1.0}
    \def\opac{100}
    \def\opaci{100}
    \def\marksz{1.5pt}

    \begin{axis}[
        width=.45\textwidth,
        height=.2\textwidth,
        xscale=1,
        xlabel=$J$,
        ylabel={$Z_\mathrm{avg}$},
        xtick = {2,4,6,8,10},
        grid=major,
        legend cell align={left},
        legend style={
            at={(0.5,1.1)},
            anchor=south,
            fill opacity = 0.8,
            draw opacity = 1, 
            text opacity = 1,
            legend columns=4,
            /tikz/every even column/.append style={column sep=.2cm}
        },
        xmin=4,xmax=10,
        ymin=0,ymax=300,
        axis line style=thick,
        tick label style={/pgf/number format/fixed},
        ]


    \addplot[color=KITcyanblue, line width=\lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax4_spikes] {figures/txt/arnold.txt};
    \addplot[color=KITorange, line width=\lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax6_spikes] {figures/txt/arnold.txt};
    \addplot[color=KITpalegreen, line width=\lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax8_spikes] {figures/txt/arnold.txt};
    \addplot[color=KITpurple, line width=\lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax10_spikes] {figures/txt/arnold.txt};
    \addplot[color=black, line width = \lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax60_spikes] {figures/txt/arnold.txt};
    \addplot[color=black, dashed, line width = \lwidth,mark=*,mark size=\marksz,mark options={solid}] table [x=nenc,y = tmax60_noopt_spikes] {figures/txt/arnold.txt};

    

    \end{axis}
\end{tikzpicture}

